Experienced Deep Reinforcement Learning with Generative Adversarial Networks (GANs) for Model-Free Ultra Reliable Low Latency Communication

In this paper, a novel experienced deep reinforcement learning (deep-RL) framework is proposed to provide model-free resource allocation for ultra reliable low latency communication (URLLC). The proposed, experienced deep-RL framework can guarantee high end-to-end reliability and low end-to-end latency, under explicit data rate constraints, for each wireless without any models of or assumptions on the users' traffic. In particular, in order to enable the deep-RL framework to account for extreme network conditions and operate in highly reliable systems, a new approach based on generative adversarial networks (GANs) is proposed. This GAN approach is used to pre-train the deep-RL framework using a mix of real and synthetic data, thus creating an experienced deep-RL framework that has been exposed to a broad range of network conditions. Formally, the URLLC resource allocation problem is posed as a power minimization problem under reliability, latency, and rate constraints. To solve this problem using experienced deep-RL, first, the rate of each user is determined. Then, these rates are mapped to the resource block and power allocation vectors of the studied wireless system. Finally, the end-to-end reliability and latency of each user are used as feedback to the deep-RL framework. It is then shown that at the fixed-point of the deep-RL algorithm, the reliability and latency of the users are near-optimal. Moreover, for the proposed GAN approach, a theoretical limit for the generator output is analytically derived. Simulation results show how the proposed approach can achieve near-optimal performance within the rate-reliability-latency region, depending on the network and service requirements. The results also show that the proposed experienced deep-RL framework is able to remove the transient training time that makes conventional deep-RL methods unsuitable for URLLC.

==> TCOM Deep RL Revision 1 (Version 1078)/acronyms.tex <==
\newacro{drl}[deep-RL]{deep reinforcement learning}
\newacro{qoe}[QoE]{quality-of-experience}
\newacro{qos}[QoS]{quality-of-service}
\newacro{gan}[GAN]{generative adversarial network}
\newacro{rb}[RB]{resource block}
\newacro{mdp}[MDP]{Markov decision process}
\newacro{ofdma}[OFDMA]{orthogonal frequency-division multiple access}
\newacro{dnn}[DNN]{deep neural network}
\newacro{bs}[BS]{base station}
\newacro{ppo}[PPO]{proximal policy optimization}
\newacro{dqn}[DQN]{deep Q-networks}
\newacro{sgd}[SGD]{stochastic gradient descent}
\newacro{urllc}[URLLC-6G]{ultra reliable low latency communication}


